Assessing the Solid Protocol in Relation to Security & Privacy Obligations

The Solid specification aims to empower data subjects by giving them direct access control over their data across multiple applications. As governments are manifesting their interest in this framework for citizen empowerment and e-government services, security and privacy represent pivotal issues to be addressed. By analyzing the relevant legislation, notably GDPR, and international standards, namely ISO/IEC 27001:2011 and 15408, we formulate the primary security and privacy requirements for such a framework. Furthermore, we survey the current Solid protocol specifications regarding how they cover the highlighted requirements, and draw attention to potential gaps between the specifications and requirements. We also point out the contribution of recent academic work presenting novel approaches to increase the security and privacy degree provided by the Solid project. This paper has a twofold contribution to improve user awareness of how Solid can help protect their data and to present possible future research lines on Solid security and privacy enhancements.

==> AttackAnalysis.tex <==
\section{Attack Defence Framework Analysis of Solid}


\todo{ give attack-tree cyber-risk assessment of current protocols.}


==> Compute.tex <==
\section{How to Compute with Data Pods Privately}


\rh{This is the section Chang Sun will rewrite. Below are some miscellaneous notes.



Use a simple running example such as calculating the \textit{average weight} of a collection of users without revealing the weight of individuals to illustrate such computation.

Push computation into the nodes.

Multi-party computation to gather analytics about groups of Solid agents. How to manage leakage, e.g., if insufficient agents participants in order to guarantee sufficient privacy.


Prospect of locally differential private learning of models, e.g., GNNs, which are representative of the data in a collection of agents, without revealing information about any individual.


What are the attacker profiles, threat models, etc.

``Accountable algorithms''~\cite{Kroll2016}


Idea: generating counter-factuals to help resolve policy violations (abduction problem):
~\cite{Wachter2018}


Collated notes from discussing with colleagues:

As far as I can see this is their current research question. Essentially, they are putting two and two together. On one hand in differential privacy in general there is a trend towards learning models of datasets that do not reveal anything about individual records~\cite{Abadi2016}. On the other hand, for graphs, the appropriate model for learning is a GNN. There are surprisingly few papers at the intersection of these topics,~\cite{Sajadmanesh2021} being perhaps the most credible for us, but still probably short of our purposes, so perhaps there is an opportunity here.

 
I can see the reason behind their thinking. For a while they worked on directly publishing anonymised social graphs ( (k,l)-anonymity, etc.~\cite{Mauw2019}, which is in line work current proposals for KGs~\cite[Section 9.3.4]{Hogan2021}), but always could find a way that a more sophisticated attacker could get around the procedures. Also the mechanisms quickly grew computationally expensive. So, now, instead of publishing an anonymised graph, they are thinking of learning and publishing a model of the graph.

This begs a few questions, for DKGs:
\begin{itemize}
\item When publishing models of private DKGs, what queries do we expect to ask? ...certainly not SPARQL queries.
\item What happens when there are hybrid distributed policies, where some private data is published directly, or with a (k,l)-anonymity applied, rather than only as a model.
\item What is the trust model for cooperating on generating models of graphs, and is it realistic/enforceable within the scope of Solid for example.
\item What are the further publish-subscribe / information flow problems due to distributed policies, which might be more heterogeneous than normally consider for "local differential privacy"~\cite{Kasiviswanathan2011}.
\end{itemize}
}


==> ContractualPolicy.tex <==
\section{A Contractual Policy Approach to Privacy in Solid}

\rh{I can develop this with a colleague working on related contractual policy problems. Ignore for now.}

We explain here approach to meeting privacy requirement where raw data is still shared with parties, but the policy which the data is subject to is made explicit. 

The Access Control Ontology can be extended to include information about the scope of requests, including their duration, and the contract under which the access is permitted. The agents should indicate, and prove their jurisdiction.


Parameters to consider:
\begin{itemize}
\item The permitted usage of the data.
\item The duration the data is available.
\item How data should be disposed of after use.
\item Managing periodic access to data that changes. 
\item The provenance information.
\item Indirect policy constraints, e.g., via data aggregation.
\item The production of machine verifiable proof of agreement, e.g., via signed timestamping or blockchain.
\item Trust issues, e.g., how can the network self-regulate information of the trustworthiness of apps and agents (e.g., as for media~\cite{Fournet2021}). 
\end{itemize}

The GPRD  becomes a consideration for Solid, given that the data in Solid is personal data. Even data that is not directly about the individual, is part of their profile in that it can be used as an indicator of their behaviour and interests, e.g., for targeted advertising purposes or for directing cyber attacks. Thus data is subject to regulation for data processing.





Legal expertise is required to determine the legal status of the contractual policy enter into when data is exchanged. Proof of contract, e.g., via timestamping/blockchain, and the status of agreements in court, e.g., in the case that a party believes the contractual terms for usage of personal data been breached, should be considered.


What are the attacker profiles, threat models, etc.

What about current initiatives, e.g., Linked Data Proofs of authenticity
https://w3c-ccg.github.io/ld-proofs/



Raw data may be shared with a trusted service that aggregates data.

$k\ell$-anonymity and associated problems. E.g., Sibyls. Question: to what extend can OpenID Connect protect against Sibyls.

What are the attacker profiles, threat models, etc.


``Realizing Purpose-Based Privacy Policies Succinctly via Information-Flow Labels''\cite{Kumar2014}



==> RelWork.tex <==
\section{Related Work}
\label{sec:academic}

\todo{
To compare to related work:

``Towards Complete Decentralised Verification of Data with
Confidentiality: Different ways to connect Solid Pods and
Blockchain''~\cite{Ramachandran2020},

``Privacy-preserving AI Services Through Data Decentralization''
~\cite{Meurisch2020}

``A Blockchain-Assisted Trust Access
Authentication System for Solid''~\cite{Cai2020}

``Greater Control and Transparency in Personal Data Processing''
~\cite{Havur2020}
}

The Solid API works by granting applications or other agents access to slices of data in a data pod,
much like data APIs for Twitter and Facebook can grant access to data in a particular scope.
